Thompson Sampling: An Asymptotically Optimal Finite Time Analysis

The question of the optimality of Thompson Sampling for solving the stochastic multi-armed bandit problem had been open since 1933. In this paper we answer it positively for the case of Bernoulli rewards by providing the first finite-time analysis that matches the asymptotic rate given in the Lai and Robbins lower bound for the cumulative regret. The proof is accompanied by a numerical comparison with other optimal policies, experiments that have been lacking in the literature until now for the Bernoulli case.

==> ConcentrationLemma.tex <==
We begin with a decomposition:
\begin{align*}
&  \bP\left(\theta_{a,s}> \mu_a + \delta_a, N_{a,s}> C_a\log(t)\right) \\
&  \leq  \bP\left(\left(\theta_{a,s}> \mu_a +{\delta_a}\right)\cap \left(\muhat_{a,s} \leq \mu_a + \frac{\delta_a}{2}\right) \cap\left(N_{a,s}> C_a\log(t)\right)\right) \\
& \ \ \  \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \  \ \ \ + \bP\left(\left(\muhat_{a,s} > \mu_a + \frac{\delta_a}{2}\right)\cap\left(N_{a,s}> C_a\log(t)\right)  \right) \\
& \leq  \underbrace{\bP\left(\left(\theta_{a,s}> \muhat_{a,s} + \frac{\delta_a}{2} \right) \cap\left(N_{a,s}> C_a\log(t)\right)\right)}_C + \underbrace{\bP\left(\left(\muhat_{a,s} > \mu_a + \frac{\delta_a}{2}\right)\cap\left(N_{a,s}> C_a\log(t)\right)  \right)}_D 
\end{align*}

For term (D), we use an union bound, writing $L=C_a\log(t)$:
$$\bP\left(\left(\muhat_{a,s} > \mu_a + \frac{\delta_a}{2}\right)\cap\left(N_{a,s}> L \right)  \right) \leq \bP\left(\exists r\in \{L,\dots, s\}\left(\frac{S_{a,r}}{r} > \mu_a + \frac{\delta_a}{2}\right)  \right)$$
where $S_{a,r}$ is a sum of the first $r$ rewards from arm $a$ (binomial with parameters $j$ and $\mu_a$). Then:
\begin{align*}
&\bP\left(\left(\muhat_{a,s} > \mu_a + \frac{\delta_a}{2}\right)\cap\left(N_{a,s}> L\right)  \right) \leq \sum_{r = L}^{s} \bP\left(\frac{S_{a,r}}{r} > \mu_a + \frac{\delta_a}{2} \right)\\
& \underset{\text{Hoeffding}}{\leq} \sum_{r = L}^{s}e^{-2r\delta_a^2/4} \leq \sum_{r = L}^{s}e^{-2L\delta_a^2/4} \leq t e^{-2C_a\log(t) \delta_a^2/4} \leq \frac{1}{t^3} 
\end{align*}

Now for term (C),
\begin{align*}
& \bP\left(\left(\theta_{a,s}> \muhat_{a,s} + \frac{\delta_a}{2} \right) \cap\left(N_{2,s}> C_a\log(t)\right)\right) \\
& = \sum_{\tau= C_a\log(t)}^t\sum_{r \leq \tau} \bP\left(\theta_2(s)> \frac{r}{\tau} + \frac{\delta_a}{2} \mid \muhat_{a,s}N_{a,s}=r, N_{a,s}=\tau \right) \bP\left(\muhat_{a,s}N_{a,s}=r, N_{a,s}=\tau\right) \\
& = \sum_{\tau= C_a\log(t)}^t\sum_{r \leq \tau}\exp\left(-2\tau {\delta_a^2}/{4}\right) \bP\left(\muhat_{a,s}N_{a,s}=r, N_{a,s}=\tau\right) \leq e^{-2C_a\log(t) \delta_a^2/4} \leq \frac{1}{t^4} 
\end{align*}
which concludes the proof.
